Double-Bracket Algorithmic Cooling

Algorithmic cooling shows that it is possible to locally reduce the entropy of a qubit belonging to an isolated ensemble such as nuclear spins in molecules or nitrogen-vacancy centers in diamonds. In the same physical setting, we introduce double-bracket algorithmic cooling (DBAC), a protocol that systematically suppresses quantum coherence of pure states. DBAC achieves this by simulating quantum imaginary-time evolution through recursive unitary synthesis of Riemannian steepest-descent flows and it utilizes density-matrix exponentiation as a subroutine. This subroutine makes DBAC a concrete instance of a dynamic quantum algorithm that operates using quantum information stored in copies of the input states. Thus, the circuits of DBAC are independent of the input state, enabling the extension of algorithmic cooling from targeting entropy to quantum coherence without resorting to measurements. Akin to Nernst principle, DBAC increases the cooling performance when including more input qubits which serve as quantum instructions. Our work demonstrates that dynamic quantum algorithms are a promising route toward new protocols for foundational tasks in quantum thermodynamics.

==> oblivious_purification.tex <==
\section{Oblivious purity amplification}
Ref.~\cite{Cirac1999_purification} introduced a probabilistic protocol, which we will refer to as interferential mixedness reduction.
In Lemma~\ref{lemma:purification}, we present this protocol along with the proof, using notation that explicitly incorporates the mixedness parameter.
Afterwards, in Proposition~\ref{pro:mixedness_reduction_subroutine}, we analyze the success probability of the mixedness reduction subroutine, which arises from using rounds of interferential mixedness reduction.
%Finally, the overall overhead required for the mixedness reduction is assessed in Proposition~\ref{pro:overhead_mixedness_reduction}.

\begin{lem}[Interferential mixedness reduction~\cite{Cirac1999_purification}]\label{lemma:purification}
Let $ \rho = (1-x)\psi + x\frac{\1_{\rm rel}}{2}$ be a state with mixedness parameter $x\in [0,1)$.
Using a controlled swap operation on the two-copy state $\rho^{\otimes 2}$, a purer state $ \rho' = (1-x')\psi + x'\frac {\1_{\rm rel}}2 $ with mixedness parameter $ x' = \frac{2+x}{4-2x+x^{2}}x $ can be prepared with success probability $ (1-\frac{x}{2}+\frac{x^{2}}{4}) $.
The procedure is oblivious, i.e. no knowledge of the state $ \psi $ or the subspace $ \mH_{\rm rel} $ is required. 
\end{lem}
\begin{proof}
	Following~\cite{Cirac1999_purification}, any two copies of a rank-2 state $ \rho \in\mS_{\rm rel}$ can be written as
	\begin{align}\label{key}
		\rho^{\otimes 2} = \frac{2x-x^{2}}{4}\Psi^{-}_{12} + \left(\frac{x^{2}}{4}\psi^{\perp}\otimes\psi^{\perp} + \frac{2x-x^{2}}{4}\Psi^{+}_{12} + \frac{(2-x)^{2}}{4}\psi\otimes\psi\right)\ ,
	\end{align}
	where $ \psi^{\perp}\in\mS_{\rm rel} $ is a pure state orthonormal to $ \psi $ and $ \Psi^{\pm}_{12} = \dm{\Psi^{\pm}}_{12} $ are Bell states, such that $ \ket{\Psi^{\pm}}_{12} = \frac{1}{\sqrt{2}}(\ket{\psi\psi^{\perp}}_{12} \pm \ket{\psi^{\perp}\psi}_{12}) $. 
	Subscripts $ 1 $ and $ 2 $ denote the space each copy of $ \rho $ lives in. 
	The main protocol is to apply the projector $ \frac{\1_{12}+S_{12}}{2} $, where $ \1_{12} $ is the identity on the total space of two copies and $ S_{12} $ is a swap between the first and the second copies. 
	Note that 
  
	\begin{align}
		\frac{\1_{12}+S_{12}}{2} = \psi^{\perp}\otimes\psi^{\perp} + \Psi^{+}_{12} + \psi\otimes\psi\ , 
	\end{align}
	after which $ \Psi^{-}_{12} $ component will vanish from the state $ \rho^{\otimes 2} $. 
	This operation can be implemented by a linear combination of unitaries utilizing an additional ancilla qubit $ \ket{0}_{A} $~\cite{Childs2012LCU}, since both $ \1_{12} $ and $ S_{12} $ are unitaries. 
	To a state $ \dm{0}_{A}\otimes \rho^{\otimes 2} $ appended with ancilla, apply a unitary 
	\begin{align}
		U &= \left(H_{A}\otimes\1_{12}\right)\left(\dm{0}_{A}\otimes \1_{12} + \dm{1}_{A}\otimes S_{12}\right) \left(H_{A}\otimes\1_{12}\right)\nonumber \\&= \left(\dm{0}_{A}+\dm{1}_{A}\right)\otimes\frac{\1_{12}+S_{12}}{2} + \left(\ketbra{1}{0}_{A}+\ketbra{0}{1}_{A}\right)\otimes\frac{\1_{12}-S_{12}}{2} \ ,
	\end{align} 
	by concatenating Hadamard operators $ H_{A} $ acting on the ancilla and a controlled swap operation, applying the swap $ S_{12} $ between two copies conditioned on the ancilla state $ \ket{1} $.
	After this operation, the ancilla plus system state becomes
	\begin{align}
		U\left(\dm{0}_{A}\otimes \rho^{\otimes 2}\right)U^{\dagger} = &\dm{0}_{A}\otimes \left(\frac{\1_{12}+S_{12}}{2}\right)\rho^{\otimes 2}\left(\frac{\1_{12}+S_{12}}{2}\right) + \dm{1}_{A}\otimes \left(\frac{\1_{12}-S_{12}}{2}\right)\rho^{\otimes 2}\left(\frac{\1_{12}-S_{12}}{2}\right)\nonumber\\
		&+\left[ \ketbra{1}{0}_{A}\otimes\left(\frac{\1_{12}-S_{12}}{2}\right)\rho^{\otimes 2}\left(\frac{\1_{12}+S_{12}}{2}\right)+ \mathrm{h.c.}\right]\ .
	\end{align}
	By measuring the ancilla in $ \{\ket{0}_{A},\ket{1}_{A}\} $ basis, we effectively achieve (unnormalized) system states 
	\begin{align}
		\begin{cases}
			\frac{x^{2}}{4}\psi^{\perp}\otimes\psi^{\perp} + \frac{2x-x^{2}}{4}\Psi^{+}_{12} + \frac{(2-x)^{2}}{4}\psi\otimes\psi\ ,\quad &\text{if $ \ket{0}_{A} $ is measured,}\\
			\frac{2x-x^{2}}{4}\Psi^{-}_{12}\ , \quad &\text{if $ \ket{1}_{A} $ is measured,}
		\end{cases}
	\end{align}
	with probability given by their traces, $ 1-\frac{x}{2}+\frac{x^{2}}{4} $ and $ \frac{2x-x^{2}}{4} $, respectively.
	For our purpose, the protocol is successful when $ \ket{0}_{A} $ is measured, in which case the normalized density matrix
	\begin{align}\label{key}
		\Omega_{12} = \frac{4}{4-2x+x^{2}}\left(\frac{x^{2}}{4}\psi^{\perp}\otimes\psi^{\perp} + \frac{2x-x^{2}}{4}\Psi^{+}_{12} + \frac{(2-x)^{2}}{4}\psi\otimes\psi\right)
	\end{align}
	remains. 
	The reduced state from $ \Omega_{12} $ for both subsystems are the same and given as
	\begin{align}\label{key}
		\rho' \coloneq \tr_{1}\left[\Omega_{12}\right] = \tr_{2}\left[\Omega_{12}\right] =  (1-x')\psi + x'\frac{\1_{\rm rel}}{2},
	\end{align}
	with $ x' = \frac{2+x}{4-2x+x^{2}}x <x $. 
	The correlation between two subsystems in $ \Omega_{12} $ might play a destructive role in our algorithm. 
	Hence, we discard one of the copies and take only a single reduced state $ \rho' $. 
\end{proof}
When $ x\ll 1 $, the success probability is close to $ 1 $ and $ x' = \frac{x}{2} + \mO(x^{2}) $, i.e. we efficiently reduce the mixedness by just consuming copies of the same state, without changing the pure part $ \psi $ of that state. 
Another merit of doing this subroutine is that we can estimate $ x $ and thus $ x' $ by the success probability, which can be used to improve the process in Lemma~\ref{lem:mixed_step} by modifying angles $\{s_{l}\}$ in $ \hE{s_{l}}{\rho} $ according to the estimated value of mixedness parameter.
Nevertheless, we restrict ourselves to the case where $ x $ is completely unknown apart from its upper bound for simplicity of analysis. 
